ST-KeyS: Self-Supervised Transformer for Keyword Spotting in Historical Handwritten Documents

Keyword spotting (KWS) in historical documents is an important tool for the initial exploration of digitized collections. Nowadays, the most efficient KWS methods are relying on machine learning techniques that require a large amount of annotated training data. However, in the case of historical manuscripts, there is a lack of annotated corpus for training. To handle the data scarcity issue, we investigate the merits of the self-supervised learning to extract useful representations of the input data without relying on human annotations and then using these representations in the downstream task. We propose ST-KeyS, a masked auto-encoder model based on vision transformers where the pretraining stage is based on the mask-and-predict paradigm, without the need of labeled data. In the fine-tuning stage, the pre-trained encoder is integrated into a siamese neural network model that is fine-tuned to improve feature embedding from the input images. We further improve the image representation using pyramidal histogram of characters (PHOC) embedding to create and exploit an intermediate representation of images based on text attributes. In an exhaustive experimental evaluation on three widely used benchmark datasets (Botany, Alvermann Konzilsprotokolle and George Washington), the proposed approach outperforms state-of-the-art methods trained on the same datasets.

==> highlights.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%Highlights%%%%%%%%%%%%%%


- A self-supervised approach based on vision transformers for keyword spotting. 
- Learning useful representations from unlabeled data using a masked auto-encoder.
- Improving feature embedding using a two-stage downstream task based on siamese and PHOC.
- The proposed approach outperforms state-of-the-art approaches on three datasets.


%We present a self-supervised approach based on vision transformers in an encoder-decoder fashion for keyword spotting in handwritten text images. 

%We present a self-supervised approach composed of pretraining and fine-tuning stages for keyword spotting in handwritten text images. 

%The proposed approach is based on vision transformers in an encoder-decoder fashion, without any dependency
on CNNs.

%The proposed approach is composed of pretraining and fine-tuning stages. 

%The pretraining stage is used to learn the most useful representations for keyword spotting without the need of any labeled data.

%The fine-tuning stage is a two-stage downstream task based on siamese neural networks and PHOC attributes. It is used to further promote the representation and makes it more powerful in retrieving the best matching images of a given query image.

%the proposed approach deals with data variability and data scarcity issues. 

%The proposed approach is evaluated on three benchmark datasets. It achieves competitive results with the state-of-the-art. 


%• We present a deep learning framework based on Generative Adversarial Network  for document image binarization.

%• The proposed model performs document enhancement and binarization. It integrates a handwriting text recognition engine within its architecture to ensure the text readability during the enhancement process. 

 
%• The proposed model restores different forms of degradation, independently of the document language.
 
%• The proposed model is evaluated on the public H-DIBCO dataset (2018) and achieves new state-of-the-art performance.
%%%%%%%%%%%%%%%%%%%%%%%%%%end Highlights%%%%%%%%%%%%%%
